Social Contract AI: Aligning AI Assistants with Implicit Group Norms

We explore the idea of aligning an AI assistant by inverting a model of users' (unknown) preferences from observed interactions. To validate our proposal, we run proof-of-concept simulations in the economic ultimatum game, formalizing user preferences as policies that guide the actions of simulated players. We find that the AI assistant accurately aligns its behavior to match standard policies from the economic literature (e.g., selfish, altruistic). However, the assistant's learned policies lack robustness and exhibit limited generalization in an out-of-distribution setting when confronted with a currency (e.g., grams of medicine) that was not included in the assistant's training distribution. Additionally, we find that when there is inconsistency in the relationship between language use and an unknown policy (e.g., an altruistic policy combined with rude language), the assistant's learning of the policy is slowed. Overall, our preliminary results suggest that developing simulation frameworks in which AI assistants need to infer preferences from diverse users can provide a valuable approach for studying practical alignment questions.

==> sections/05_social_impacts.tex <==
% While our work is at an early stage, we believe that SCAI addresses an important non-technical alignment challenge highlighted in previous work: \textit{``figuring out what the group preferences are''} \citep{leike2023proposal}. Specifically, rather than having a team of researchers write a model's content policy or ``constitution'', we propose to have an AI assistant learn group norms and preferences through observation and active participation in interactions with simulated users. This approach allows for (1) the study of the kinds of group norms that \textit{emerge} under varying conditions; (2) assessing the \textit{flexibility} of learning such group norms; and (3) studying the \textit{robustness} of group norms as guiding principles for the AI assistant, especially in out-of-distribution scenarios. In sum, scaling up a ``bottom-up'' approach such as SCAI may provide insights into designing more democratic and representative guiding norms for AI assistants \citep{zaremba2023democratic}.


